Proving Correctness of Parallel Implementations of Transition System Specifications

The overall problem addressed in this paper is the long-standing problem of program correctness, and in particular programs that describe systems of parallel executing processes. We propose a new method for proving correctness of parallel implementations of high-level transition system specifications. The implementation language underlying the method is based on the model of active (or concurrent) objects. The method defines correctness in terms of a simulation relation between the transition system which specifies the program semantics and the transition system that is described by the correctness specification. The simulation relation itself abstracts from the fine-grained interleaving of parallel processes by exploiting a global confluence property of the particular model of active objects considered in this paper. As a proof-of-concept we apply our method to the correctness of a parallel simulator of multicore memory systems.

==> ABScode.tex <==
\subsection{Core}
The   only method of class \Abs{Core} is the run method,
see figure  \ref{fig:ABScore} for its annotated implemenation.
% \input{AnnotatedABS/runcore_abs}

\subsection{Cache}
%\input{AnnotatedABS/fetch_abs}

%\input{AnnotatedABS/fetchbl_abs}

%\input{AnnotatedABS/fetchblw_abs}

%\input{AnnotatedABS/flush_abs}

%\input{AnnotatedABS/receiveRd_abs}

%\input{AnnotatedABS/receiveRdx_abs}

\input{AnnotatedABS/flush_abs}

%\input{AnnotatedABS/swap}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
